Human Interaction with Recommendation Systems

Many recommendation algorithms rely on user data to generate recommendations. However, these recommendations also affect the data obtained from future users. This work aims to understand the effects of this dynamic interaction. We propose a simple model where users with heterogeneous preferences arrive over time. Based on this model, we prove that naive estimators, i.e. those which ignore this feedback loop, are not consistent. We show that consistent estimators are efficient in the presence of myopic agents. Our results are validated using extensive simulations.

==> base/commands.tex <==
\newcommand{\eps}{\varepsilon}

\newcommand{\abs}[1]{\ensuremath{\left|#1\right|}}
\newcommand{\union}{\ensuremath{\bigcup}}
\newcommand{\eq}{{\rm eq}}

\newcommand{\comps}{\ensuremath{\mathbb{C}}}
\newcommand{\reals}{\ensuremath{\mathbb{R}}}
\newcommand{\ints}{\ensuremath{\mathbb{Z}}}

\newcommand{\diag}{\ensuremath{\operatorname{diag}}}

\newcommand{\E}{\ensuremath{\mathbb{E}}}
\renewcommand{\P}{\ensuremath{\mathbb{P}}}
\newcommand{\var}[1]{\textup{Var}\left(#1\right)}
\newcommand{\cov}[1]{\textup{Cov}\left(#1\right)}

\newcommand{\disp}[1]{\ensuremath{\displaystyle{#1}}}
\renewcommand{\epsilon}{\varepsilon}
\renewcommand{\v}[1]{\ensuremath{\boldsymbol{\mathrm{#1}}}}
\renewcommand{\b}[1]{\ensuremath{\overline{#1}}}
\newcommand{\mc}[1]{\ensuremath{\mathcal{#1}}}
\renewcommand{\Re}{\ensuremath{\operatorname{Re}}}

\newcommand{\cS}{\ensuremath{\mathcal{S}}}
\newcommand{\cB}{\ensuremath{\mathcal{B}}}
\newcommand{\cF}{\ensuremath{\mathcal{F}}}
\newcommand{\cC}{\ensuremath{\mathcal{C}}}
\newcommand{\cE}{\ensuremath{\mathcal{E}}}
\newcommand{\cO}{\ensuremath{\mathcal{O}}}
\newcommand{\co}{\ensuremath{\mathcal{o}}}
\newcommand{\cH}{\ensuremath{\mathcal{H}}}

\renewcommand{\c}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\av}{\rm{\tiny av}}
\newcommand{\uX}{{\underline{X}}}
\newcommand{\ux}{{\underline{x}}}

\newcommand{\Ev}{{\cE}}
\newcommand{\ind}{{\mathbb{I}}}
\newcommand{\Po}{\textup{Poisson}}
\newcommand{\Bern}{\textup{Bernoulli}}
\newcommand{\Binom}{\textup{Binomial}}
\newcommand{\N}{\mathcal{N}}

\newcommand{\regret}{\textup{regret}}

\providecommand{\norm}[1]{\lVert#1\rVert}
\providecommand{\abs}[1]{\lvert#1\rvert}

\newcommand{\smsp}{\vspace{0.05in}}

\newcommand{\X}{\ensuremath{\mathbf{X}}}
\newcommand{\h}{\ensuremath{\mathbf{H}}}

% \newtheorem{theorem}{Theorem}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{conjecture}[theorem]{Conjecture}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{assump}{Assumption}
% \newtheorem{fact}{Fact}
% \newtheorem{rem}{Remark}
% \newtheorem{example}{Example}
% \newtheorem{definition}{Definition}

% for auto equation numbering
\renewcommand{\[}{\begin{equation}}
\renewcommand{\]}{\end{equation}}



==> base/packages.tex <==
% \usepackage{fullpage}

% \usepackage{amsmath, amsthm} % not needed for amsart
% \usepackage{amsfonts}
% \usepackage{amssymb}
% \usepackage{amsthm}

% \usepackage[english]{babel}
\usepackage{natbib}
% \usepackage{bookmark}
\usepackage{booktabs}
\usepackage{dcolumn}

\usepackage{enumerate}

\usepackage{graphicx}
% \usepackage{tikz}
% \usetikzlibrary{shapes,arrows}

\usepackage{hyperref}
\usepackage{xr}

% \usepackage{latexsym}

% \usepackage{multirow}

% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography


% font
% \usepackage{mathptmx}
% \usepackage[scaled=.90]{helvet}
% \usepackage{courier}


==> tex/acknowledgements.tex <==
\section{Acknowledgements}
	This work is published in the proceedings of AISTATS 2018.
	The authors would like to thank Ramesh Johari, Vijay Kamble, Brad Klingenberg,
	Yonatan Gur, Peter Lofgren, Andrea Locatelli, and anonymous reviewers for their suggestions and feedback.
	This work was supported by the Stanford TomKat Center, and by the National Science Foundation under
	Grant No. CNS-1544548.  Any opinions, findings, and conclusions or recommendations expressed in this
	material are those of the author(s) and do not necessarily reflect the views of the National Science
	Foundation.


==> tex/arxiv.tex <==

\title{
    Human Interaction with Recommendation Systems
}

\author{
    Sven Schmit\thanks{schmit@stanford.edu}\\
    Stanford University
    \and
    Carlos Riquelme\thanks{rikel@google.com}\\
    Google Brain
}

\date{\today}

% \usepackage[draft]{todonotes}

% \renewcommand{\baselinestretch}{1.2}

\begin{document}

    \maketitle

    \input{tex/abstract}
    \input{tex/intro}
    \input{tex/model}
    \input{tex/bias}
    \input{tex/exploration}
    \input{tex/simulations}
    \input{tex/conclusion}

    \input{tex/acknowledgements}

    \bibliographystyle{plainnat}
    \bibliography{bib/bibliography}

    \input{tex/supplement}


\end{document}

